Learning Energy-Based Models by Self-normalising the Likelihood

Training an energy-based model (EBM) with maximum likelihood is challenging due to the intractable normalisation constant. Traditional methods rely on expensive Markov chain Monte Carlo (MCMC) sampling to estimate the gradient of logartihm of the normalisation constant. We propose a novel objective called self-normalised log-likelihood (SNL) that introduces a single additional learnable parameter representing the normalisation constant compared to the regular log-likelihood. SNL is a lower bound of the log-likelihood, and its optimum corresponds to both the maximum likelihood estimate of the model parameters and the normalisation constant. We show that the SNL objective is concave in the model parameters for exponential family distributions. Unlike the regular log-likelihood, the SNL can be directly optimised using stochastic gradient techniques by sampling from a crude proposal distribution. We validate the effectiveness of our proposed method on various density estimation tasks as well as EBMs for regression. Our results show that the proposed method, while simpler to implement and tune, outperforms existing techniques.

==> mnist_sample/mnist_image_samples.tex <==

% \begin{figure}[!h]
%     \centering
%     \setlength{\tabcolsep}{1pt} 
%     \begin{tabular}{cc}
%     % {\textbf{(A)}} & 
%     \begin{subfigure}{.45\textwidth}
%         \centering
%         \includegraphics[width=\linewidth, trim={5cm 4cm 3cm 4cm},clip]{mnist_sample/mnist_mean_VAE.png}
%     \end{subfigure} &

    % \begin{subfigure}{.45\textwidth}
    %     \centering
    %     \includegraphics[width=\linewidth, trim={5cm 4cm 3cm 4cm},clip]{mnist_sample/mnist_mean_full_prior.png}
    % \end{subfigure} 
%     \end{tabular}
%     \caption{\label{fig:mnist_sample} Continuous s }
% \end{figure}


\begin{figure}[!h]
    \begin{tabular}{cc}

    % \begin{subfigure}{.24\textwidth}
        % \centering
        % \includegraphics[width=\linewidth]{mnist_sample/mnist_mean_mixture.png}
    % \end{subfigure} &
    % \begin{subfigure}{.24\textwidth}
        % \centering
        % \includegraphics[width=\linewidth]{mnist_sample/mnist_mean_detached_prior.png}
    % \end{subfigure} &
    % {\textbf{(B)}} &
    Standard VAE  & VAE-EBM 
    \\ % Row two
       \begin{subfigure}{.45\textwidth}
        \centering
        \includegraphics[width=\linewidth, trim={5cm 4cm 3cm 4cm},clip]{mnist_sample/mnist_sample_vae.png}
    \end{subfigure} &
    % \begin{subfigure}{.24\textwidth}
        % \centering
        % \includegraphics[width=\linewidth]{mnist_sample/mnist_sample_mixture.png}
    % \end{subfigure} &
    % \begin{subfigure}{.24\textwidth}
        % \centering
        % \includegraphics[width=\linewidth]{mnist_sample/mnist_sample_detached_prior.png}
    % \end{subfigure} &
    % {\textbf{(B)}} &
    \begin{subfigure}{.45\textwidth}
        \centering
        \includegraphics[width=\linewidth, trim={5cm 4cm 3cm 4cm},clip]{mnist_sample/mnist_sample_full_prior.png}
    \end{subfigure} 
    \\
    \end{tabular}
\caption{\label{fig:mnist_sample} Samples from the VAE with gaussian prior and the VAE with EBM prior.}
\end{figure}

==> regression_data/regression_data.tex <==

\begin{figure}
    \centering
    \setlength{\tabcolsep}{1pt} 
    \begin{tabular}{cccc}
    {\textbf{(A)}} & 
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{regression_data/d1regression_1.pdf}
    \end{subfigure} &
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{regression_data/d1regression_1.pdf}
    \end{subfigure} &
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{regression_data/d1regression_1.pdf}
    \end{subfigure}\\ % Row two
    {\textbf{(B)}} &
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{regression_data/d2regression_1.pdf}
    \end{subfigure} &
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{regression_data/d2regression_1.pdf}
    \end{subfigure} &
    \begin{subfigure}{.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{regression_data/d2regression_1.pdf}
    \end{subfigure}\\ % Row three
    
    \end{tabular}
\caption{(A): Dataset regression 1. (B): Dataset regression 2.}
\end{figure}

==> table_datasets/table_maf.tex <==
% \begin{table}[]
% \caption{Tabular datasets: data dimensionality and number of training examples. This table is directly taken from \cite{kobyzev2020normalizing}.}
% \centering
% \begin{tabular}{||cccccc||}
% \hline & POWER & GAS & HEPMASS  \\
% \hline \hline Dims & 6 & 8 & 21 \\
% \hline \#Train & $\approx 1.7 \mathrm{M}$ & $\approx 800 \mathrm{~K}$ & $\approx 300 \mathrm{~K}$  \\
% \hline
% \end{tabular}

% \end{table}


==> table_results/large_table_2d.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{booktabs}
% \begin{table}[]
% \begin{adjustbox}{max width=1.1\textwidth,center}
% \label{table:2d_distribution_estimation}
% \begin{tabular}{@{}cclllllllllllll@{}}
% \multicolumn{2}{c}{Models}                                                         &  & \multicolumn{12}{c}{Datasets}                                                                                                                                                                                                                                                                                                                                                                                                 \\ \cmidrule(r){1-2} \cmidrule(l){4-15} 
% \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                                        &  & \multicolumn{3}{c}{Funnel}                                                                            & \multicolumn{3}{c}{Pinwheel}                                                                          & \multicolumn{3}{c}{Checkerboard}                                                                      & \multicolumn{3}{c}{Four Circles}                                                                      \\ \cmidrule(l){4-15} 
% Objective            & \begin{tabular}[c]{@{}c@{}}Base\\ Distribution\end{tabular} &  & \multicolumn{1}{c}{$\ell_{\text{IS}}$} & \multicolumn{1}{c}{$\ell_{\text{SNL}}$} & $\log{Z_{\theta}}$ & \multicolumn{1}{c}{$\ell_{\text{IS}}$} & \multicolumn{1}{c}{$\ell_{\text{SNL}}$} & $\log{Z_{\theta}}$ & \multicolumn{1}{c}{$\ell_{\text{IS}}$} & \multicolumn{1}{c}{$\ell_{\text{SNL}}$} & $\log{Z_{\theta}}$ & \multicolumn{1}{c}{$\ell_{\text{IS}}$} & $\ell_{\text{SNL}}$ & \multicolumn{1}{c}{$\log{Z_{\theta}}$} \\ \cmidrule(r){1-2} \cmidrule(l){4-15} 
% NCE                  & $\mathcal{N}(\mathbf{0}, \mathbf{1})$                                                         &  &    $-2.040$ \tiny{($\pm 0.251$)} &  $-2.044$ \tiny{($\pm 0.254$)} &  $0.078$ \tiny{($\pm 0.052$)} &  $-1.004$ \tiny{($\pm 0.072$)} &  $-1.020$ \tiny{($\pm 0.084$)} &  $0.158$ \tiny{($\pm 0.072$)} &  $-1.947$ \tiny{($\pm 0.033$)} &  $-1.964$ \tiny{($\pm 0.032$)} &  $0.167$ \tiny{($\pm 0.082$)} &  $-2.117$ \tiny{($\pm 0.005$)} &  $-2.120$ \tiny{($\pm 0.006$)} &  $0.047$ \tiny{($\pm 0.069$)}   
%  \\
% SNL                  & $\mathcal{N}(\mathbf{0}, \mathbf{1})$                                                         &  &  $-1.811$ \tiny{($\pm 0.175$)} &  $-1.831$ \tiny{($\pm 0.181$)} &  $0.063$ \tiny{($\pm 0.230$)} &  $-1.031$ \tiny{($\pm 0.066$)} &  $-1.035$ \tiny{($\pm 0.065$)} &  $0.058$ \tiny{($\pm 0.076$)} &  $-1.902$ \tiny{($\pm 0.012$)} &  $-1.905$ \tiny{($\pm 0.012$)} &  $-0.033$ \tiny{($\pm 0.071$)} &  $-1.914$ \tiny{($\pm 0.022$)} &  $-1.918$ \tiny{($\pm 0.022$)} &  $-0.029$ \tiny{($\pm 0.098$)}  
%   \\
% DSM                  & $\mathcal{N}(\mathbf{0}, \mathbf{1})$                                                         &  &   $-2.859$ \tiny{($\pm 0.212$)} &  $-2.859$ \tiny{($\pm 0.212$)} &  $-0.008$ \tiny{($\pm 0.014$)} &  $-2.839$ \tiny{($\pm 0.016$)} &  $-2.839$ \tiny{($\pm 0.017$)} &  $-0.006$ \tiny{($\pm 0.015$)} &  $-2.830$ \tiny{($\pm 0.006$)} &  $-2.830$ \tiny{($\pm 0.006$)} &  $-0.015$ \tiny{($\pm 0.009$)} &  $-2.840$ \tiny{($\pm 0.022$)} &  $-2.840$ \tiny{($\pm 0.022$)} &  $-0.003$ \tiny{($\pm 0.005$)}  
%    \\
% SM                   & $\mathcal{N}(\mathbf{0}, \mathbf{1})$                                                         &  &   $-3.298$ \tiny{($\pm 0.151$)} &  $-5.137$ \tiny{($\pm 0.392$)} &  $1.452$ \tiny{($\pm 0.113$)} &  $-3.122$ \tiny{($\pm 0.031$)} &  $-7.533$ \tiny{($\pm 0.407$)} &  $2.002$ \tiny{($\pm 0.059$)} &  $-3.104$ \tiny{($\pm 0.026$)} &  $-7.001$ \tiny{($\pm 0.511$)} &  $1.916$ \tiny{($\pm 0.084$)} &  $-3.156$ \tiny{($\pm 0.008$)} &  $-6.932$ \tiny{($\pm 0.198$)} &  $1.898$ \tiny{($\pm 0.035$)}     \\
% NCE                  & No                                                          &  &    $-1.894$ \tiny{($\pm 0.096$)} &  $-1.896$ \tiny{($\pm 0.097$)} &  $0.033$ \tiny{($\pm 0.043$)} &  $-1.063$ \tiny{($\pm 0.019$)} &  $-1.069$ \tiny{($\pm 0.024$)} &  $0.045$ \tiny{($\pm 0.113$)} &  $-1.997$ \tiny{($\pm 0.022$)} &  $-2.025$ \tiny{($\pm 0.056$)} &  $0.182$ \tiny{($\pm 0.146$)} &  $-2.231$ \tiny{($\pm 0.038$)} &  $-2.232$ \tiny{($\pm 0.039$)} &  $0.011$ \tiny{($\pm 0.036$)}   
%  \\
% SNL                  & No                                                          &  &    $-2.006$ \tiny{($\pm 0.378$)} &  $-2.066$ \tiny{($\pm 0.468$)} &  $0.226$ \tiny{($\pm 0.257$)} &  $-1.072$ \tiny{($\pm 0.040$)} &  $-1.086$ \tiny{($\pm 0.030$)} &  $-0.002$ \tiny{($\pm 0.192$)} &  $-1.966$ \tiny{($\pm 0.030$)} &  $-1.969$ \tiny{($\pm 0.028$)} &  $-0.012$ \tiny{($\pm 0.083$)} &  $-1.971$ \tiny{($\pm 0.047$)} &  $-1.973$ \tiny{($\pm 0.048$)} &  $0.027$ \tiny{($\pm 0.044$)}  
%  \\
% DSM                  & No    & &  $-4.278$ \tiny{($\pm 0.106$)} &  $-4.341$ \tiny{($\pm 0.161$)} &  $0.084$ \tiny{($\pm 0.385$)} &  $-4.278$ \tiny{($\pm 0.106$)} &  $-4.341$ \tiny{($\pm 0.161$)} &  $0.084$ \tiny{($\pm 0.385$)} &  $-4.278$ \tiny{($\pm 0.105$)} &  $-4.392$ \tiny{($\pm 0.253$)} &  $0.153$ \tiny{($\pm 0.466$)} &  $-4.278$ \tiny{($\pm 0.105$)} &  $-4.384$ \tiny{($\pm 0.258$)} &  $0.155$ \tiny{($\pm 0.443$)}  
%  \\
% SM                   & No                                                          &  &     $-4.216$ \tiny{($\pm 0.034$)} &  $-4.258$ \tiny{($\pm 0.049$)} &  $0.011$ \tiny{($\pm 0.338$)} &  $-4.216$ \tiny{($\pm 0.034$)} &  $-4.258$ \tiny{($\pm 0.049$)} &  $0.011$ \tiny{($\pm 0.338$)} &  $-4.216$ \tiny{($\pm 0.034$)} &  $-4.292$ \tiny{($\pm 0.094$)} &  $0.089$ \tiny{($\pm 0.411$)} &  $-4.216$ \tiny{($\pm 0.034$)} &  $-4.284$ \tiny{($\pm 0.100$)} &  $0.092$ \tiny{($\pm 0.384$)}   
%   \\ \cmidrule(r){1-2} \cmidrule(l){4-15} 
% \end{tabular}
% \end{adjustbox}
% \end{table}

==> table_results/large_table_uci.tex <==
% \begin{table}[]
% \label{table:uci_distribution estimation}

% \begin{adjustbox}{max width=1.1\textwidth,center}
% \begin{tabular}{clcllllllllll}
% \multicolumn{3}{c}{Models}                                                                                      &  & \multicolumn{1}{c}{Datasets}           &                                         &                    &                                        &                                         &                    &                                        &                                         &                    \\ \cline{1-3} \cline{5-13} 
% \multicolumn{1}{l}{} &                            & \multicolumn{1}{l}{}                                        &  & \multicolumn{3}{c}{Gas}                                                                               & \multicolumn{3}{c}{Hepmass}                                                                           & \multicolumn{3}{c}{Power}                                                                             \\ \cline{5-13} 
% Objective            & Proposal                   & \begin{tabular}[c]{@{}c@{}}Base\\ Distribution\end{tabular} &  & \multicolumn{1}{c}{$\ell_{\text{IS}}$} & \multicolumn{1}{c}{$\ell_{\text{SNL}}$} & $\log{Z_{\theta}}$ & \multicolumn{1}{c}{$\ell_{\text{IS}}$} & \multicolumn{1}{c}{$\ell_{\text{SNL}}$} & $\log{Z_{\theta}}$ & \multicolumn{1}{c}{$\ell_{\text{IS}}$} & \multicolumn{1}{c}{$\ell_{\text{SNL}}$} & $\log{Z_{\theta}}$ \\ \cline{1-3} \cline{5-13} 
% NCE                  & KDE                        & No                                                          &  &     $0.314$ \tiny[($\pm 0.346$)] &  $-0.282$ \tiny[($\pm 0.011$)] &  $-1.308$ \tiny[($\pm 0.457$)] &       $-22.555$ \tiny[($\pm 0.968$)] &  $-24.589$ \tiny[($\pm 4.322$)] &  $1.040$ \tiny[($\pm 0.937$)] &                $-0.651$ \tiny[($\pm nan$)] &  $-2.500$ \tiny[($\pm nan$)] &  $1.461$ \tiny[($\pm nan$)]           \\
% NCE                  & $\mathcal{N}(\mu, \Sigma)$ & No                                                          &  &   $2.732$ \tiny[($\pm 2.435$)] &  $0.167$ \tiny[($\pm 0.165$)] &  $-3.479$ \tiny[($\pm 2.383$)] &   $-20.966$ \tiny[($\pm 1.394$)] &  $-27.812$ \tiny[($\pm 14.007$)] &  $1.449$ \tiny[($\pm 1.340$)] &   $-0.178$ \tiny[($\pm nan$)] &  $-0.444$ \tiny[($\pm nan$)] &  $0.651$ \tiny[($\pm nan$)]            \\
% NCE                  & $\mathcal{N}(\mu, \Sigma)$ & $q$                                                         &  &        $1.914$ \tiny[($\pm 1.997$)] &  $-0.488$ \tiny[($\pm 0.140$)] &  $-3.307$ \tiny[($\pm 1.974$)] &      $-20.869$ \tiny[($\pm 0.630$)] &  $-21.052$ \tiny[($\pm 0.814$)] &  $0.320$ \tiny[($\pm 0.502$)] &   $-0.780$ \tiny[($\pm nan$)] &  $-1.188$ \tiny[($\pm nan$)] &  $0.785$ \tiny[($\pm nan$)]              \\
% SNL                  & KDE                        & No                                                          &  &       $0.522$ \tiny[($\pm 0.704$)] &  $-0.859$ \tiny[($\pm 0.523$)] &  $-2.256$ \tiny[($\pm 0.658$)] &     $-23.987$ \tiny[($\pm 0.220$)] &  $-24.163$ \tiny[($\pm 0.227$)] &  $-0.576$ \tiny[($\pm 0.420$)] &   $-1.143$ \tiny[($\pm nan$)] &  $-1.148$ \tiny[($\pm nan$)] &  $0.104$ \tiny[($\pm nan$)]           \\
% SNL                  & $\mathcal{N}(\mu, \Sigma)$ & No                                                          &  &                                        &                                         &                    &                                        &                                         &                    &                                        &                                         &                    \\
% SNL                  & $\mathcal{N}(\mu, \Sigma)$ & $q$                                                         &  &                                        &                                         &                    &                                        &                                         &                    &                                        &                                         &                    \\ \cline{1-3} \cline{5-13} 
% \end{tabular}
% \end{adjustbox}
% \end{table}

==> table_results/table_uci.tex <==
\begin{table}[]
\label{table:uci_distribution estimation}

\begin{adjustbox}{max width=1.1\textwidth,center}
\begin{tabular}{clcllllllllll}
\multicolumn{3}{c}{Models}                                                                                      &  & \multicolumn{1}{c}{Datasets}           &                                         &                    &                                        &                                         &                    &                                        &                                         &                    \\ \cline{1-3} \cline{5-13} 
\multicolumn{1}{l}{} &                            & \multicolumn{1}{l}{}                                        &  & \multicolumn{3}{c}{Gas}                                                                               & \multicolumn{3}{c}{Hepmass}                                                                           & \multicolumn{3}{c}{Power}                                                                             \\ \cline{5-13} 
Objective            & Proposal                   & \begin{tabular}[c]{@{}c@{}}Base\\ Distribution\end{tabular} &  & \multicolumn{1}{c}{$\ell_{\text{IS}}$} & \multicolumn{1}{c}{$\ell_{\text{SNL}}$} & $\log{Z_{\theta}}$ & \multicolumn{1}{c}{$\ell_{\text{IS}}$} & \multicolumn{1}{c}{$\ell_{\text{SNL}}$} & $\log{Z_{\theta}}$ & \multicolumn{1}{c}{$\ell_{\text{IS}}$} & \multicolumn{1}{c}{$\ell_{\text{SNL}}$} & $\log{Z_{\theta}}$ \\ \cline{1-3} \cline{5-13} 
NCE                  & KDE                        & No                                                          &  &     $0.314$ \tiny[($\pm 0.346$)] &  $-0.282$ \tiny[($\pm 0.011$)] &  $-1.308$ \tiny[($\pm 0.457$)] &       $-22.555$ \tiny[($\pm 0.968$)] &  $-24.589$ \tiny[($\pm 4.322$)] &  $1.040$ \tiny[($\pm 0.937$)] &                $-0.651$ \tiny[($\pm nan$)] &  $-2.500$ \tiny[($\pm nan$)] &  $1.461$ \tiny[($\pm nan$)]           \\
NCE                  & $\mathcal{N}(\mu, \Sigma)$ & No                                                          &  &   $2.732$ \tiny[($\pm 2.435$)] &  $0.167$ \tiny[($\pm 0.165$)] &  $-3.479$ \tiny[($\pm 2.383$)] &   $-20.966$ \tiny[($\pm 1.394$)] &  $-27.812$ \tiny[($\pm 14.007$)] &  $1.449$ \tiny[($\pm 1.340$)] &   $-0.178$ \tiny[($\pm nan$)] &  $-0.444$ \tiny[($\pm nan$)] &  $0.651$ \tiny[($\pm nan$)]            \\
NCE                  & $\mathcal{N}(\mu, \Sigma)$ & $q$                                                         &  &        $1.914$ \tiny[($\pm 1.997$)] &  $-0.488$ \tiny[($\pm 0.140$)] &  $-3.307$ \tiny[($\pm 1.974$)] &      $-20.869$ \tiny[($\pm 0.630$)] &  $-21.052$ \tiny[($\pm 0.814$)] &  $0.320$ \tiny[($\pm 0.502$)] &   $-0.780$ \tiny[($\pm nan$)] &  $-1.188$ \tiny[($\pm nan$)] &  $0.785$ \tiny[($\pm nan$)]              \\
SNL                  & KDE                        & No                                                          &  &       $0.522$ \tiny[($\pm 0.704$)] &  $-0.859$ \tiny[($\pm 0.523$)] &  $-2.256$ \tiny[($\pm 0.658$)] &     $-23.987$ \tiny[($\pm 0.220$)] &  $-24.163$ \tiny[($\pm 0.227$)] &  $-0.576$ \tiny[($\pm 0.420$)] &   $-1.143$ \tiny[($\pm nan$)] &  $-1.148$ \tiny[($\pm nan$)] &  $0.104$ \tiny[($\pm nan$)]           \\
SNL                  & $\mathcal{N}(\mu, \Sigma)$ & No                                                          &  &                                        &                                         &                    &                                        &                                         &                    &                                        &                                         &                    \\
SNL                  & $\mathcal{N}(\mu, \Sigma)$ & $q$                                                         &  &                                        &                                         &                    &                                        &                                         &                    &                                        &                                         &                    \\ \cline{1-3} \cline{5-13} 
\end{tabular}
\end{adjustbox}
\end{table}
